Resolving Symmetry Ambiguity in Correspondence-based Methods for Instance-level Object Pose Estimation

Estimating the 6D pose of an object from a single RGB image is a critical task that becomes additionally challenging when dealing with symmetric objects. Recent approaches typically establish one-to-one correspondences between image pixels and 3D object surface vertices. However, the utilization of one-to-one correspondences introduces ambiguity for symmetric objects. To address this, we propose SymCode, a symmetry-aware surface encoding that encodes the object surface vertices based on one-to-many correspondences, eliminating the problem of one-to-one correspondence ambiguity. We also introduce SymNet, a fast end-to-end network that directly regresses the 6D pose parameters without solving a PnP problem. We demonstrate faster runtime and comparable accuracy achieved by our method on the T-LESS and IC-BIN benchmarks of mostly symmetric objects. Our source code will be released upon acceptance.

==> Table/network_size.tex <==
\begin{table}[t]
        \centering
        \caption{
                The size of our network
        }
        \begin{tabular}{l c l c}
        \toprule
        backbone&21.3M&ASPPGeoNet&7.8M \\
        ConPnPnet&34.1M& Total & 63.2M \\
        \bottomrule
        \end{tabular}
\label{tab:network_size}
\end{table}


==> Table/ycbv_auc.tex <==
\begin{table}
  \centering
  \begin{tabular}{@{}l|c|c|c@{}}
    \toprule
     Method & ADD(-S) & \makecell{AUC of\\ADD-S} & \makecell{AUC of\\ADD(-S)} \\
    \midrule
    SegDriven\cite{2019segmentation} & 39.0 &  - &  -  \\
    SingleStage\cite{hu2020single} & 53.9 &  - &  - \\
    CosyPose~\cite{labbe2020cosypose} & - &  89.8 &  84.5 \\
    RePose~\cite{iwase2021repose} & 62.1 &  88.5 &  82.0 \\
    GDR-Net~\cite{wang2021gdr} & 60.1 & 91.6 &  84.4 \\
    SO-Pose~\cite{di2021so} & 56.8 &  90.9 &  83.9 \\
    ZebraPose~\cite{su2022zebrapose} & 80.5 &  90.1 & 85.3  \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Comparison on YCB-V}. We compare with state of the art w.r.t ADD(-S), AUC of ADD(-S) and AUC of ADD-S in \%. (-) denotes results missing from the original paper.}
  \label{tab:ycbv_results_table}
\end{table}

==> Table/ycbv_bop.tex <==
\begin{table*}[t]
        \centering
        \caption{
                Table 1. BOP results on dataset YCB-V.
        }
        \begin{tabular}{l c c c c c c c c}
        \toprule
        6D object pose estimation method &Input type&Training type&$AR$&$AR_{VSD}$&$AR_{MSSD}$&$AR_{MSPD}$&Time(s)\\       %表格第一行，&的位置对齐
        \midrule
        CDPNv2&RGB&pbr&0.532&0.396&0.570&0.631&0.143 \\
        EPOS&RGB&pbr&0.499&0.411&0.464&0.621&0.764 \\
        SurfEmb&RGB&pbr&0.647&0.548&0.620&0.773&5.427 \\
        ZebraPoseSAT-EffnetB4&RGB&pbr&0.691&0.607&0.686&0.780&0.25 \\
        Symnet(Ours)&RGB&pbr&0.653&0.557&0.646&0.758&0.085 \\
        \bottomrule
        \end{tabular}
\vspace{-0.05in}
\label{tab:ycbv_bop}
\end{table*}

